Automatic Root Cause Analysis via Large Language Models for Cloud Incidents

Ensuring the reliability and availability of cloud services necessitates efficient root cause analysis (RCA) for cloud incidents. Traditional RCA methods, which rely on manual investigations of data sources such as logs and traces, are often laborious, error-prone, and challenging for on-call engineers. In this paper, we introduce RCACopilot, an innovative on-call system empowered by the large language model for automating RCA of cloud incidents. RCACopilot matches incoming incidents to corresponding incident handlers based on their alert types, aggregates the critical runtime diagnostic information, predicts the incident's root cause category, and provides an explanatory narrative. We evaluate RCACopilot using a real-world dataset consisting of a year's worth of incidents from Microsoft. Our evaluation demonstrates that RCACopilot achieves RCA accuracy up to 0.766. Furthermore, the diagnostic information collection component of RCACopilot has been successfully in use at Microsoft for over four years.

==> rebuttal.tex <==
Thanks for the detailed reviews! Our response to your concerns is outlined below. 
 
\textbf{Q1: Novelty [\#A,\#D,\#E]}
 
Our novelty is a practical, end-to-end solution where the information collection module can enable efficient incident data collection (Table 4 in appendix) from heterogeneous sources, and LLMs in the prediction stage provide a promise in reasoning the incident root cause. 
 
We do not simply `plug in' an existing LLM into an on-call system and let LLM directly do the incident reasoning. Instead, we design a novel way of prompting LLM to perform the root cause analysis under the cloud incident context. 
While CoT prompting is not our innovation, its application in the context and how to automatically construct the prompt (i.e., selecting the historical incidents and their root cause categories) to form the reasoning chains are unique and, we believe, innovative.
 
We reveal a key opportunity: that is, due to the nature of heterogeneous and hard-to-understand incident information, we can 1) enable OCEs to create incident handlers to collect multi-source incident information automatically and efficiently, and 2) fill the gap between incident information and incident root cause understanding via leveraging LLMs.
 
 
 
\textbf{Q2: Production rolling of LLMs and its evaluation [\#A,\#B,\#E]}
 
 
We have deployed the LLM part of Owl in production for more than one month in our service. It has successfully detected 35 (out of 55) incidents' root cause categories and provided explanations for them. These results not only give OCEs a better understanding of the incident but also help to re-delegate incident tickets to other teams who own the corresponding buggy service. We'll include more details on how LLMs have impacted OCE's efficiency in real-world scenarios, e.g., statistics on the incident TTM (Time-to-mitigate) or user study, and show more comprehensive post-experience after using the Owl in our company. 
 
 
\textbf{Q3: Baseline details [\#B,\#C]}
 
We use the source code (Python libraries) from the original authors for XGBoost and FastText. We use 490 (75\%) incidents as training data. We use the grid to do the hyperparameter optimization. For fine-tuned GPT, it does not have a prompt design (i.e., CoT prompting) like Owl but directly predicts the category with the original diagnosis information. GPT-4 Prompt does not do training, and only the incident being predicted is in its prompt, which means there is no CoT prompting (historical incidents) in GPT-4 Prompt. GPT-4 Embed uses training data to do the GPT-4 embedding.
 
 
\textbf{Q4: Incident handler [\#D]}
 
We admit that it is common to automatically collect diagnostic information when an incident occurs.
 
However, Owl provides a platform to enable OCEs to build handler actions that can be reused across different teams for different business purposes. 
Besides, Owl's incident handlers can be updated and modified dynamically by OCEs, allowing them to stay abreast with the most recent system changes. The incident handlers are highly customizable. Users can easily delete/insert/modify an action node from the handler. 
We will clarify this clearer in the paper.
 
 
\textbf{Q5. Handler construction experience and evolution over time [\#B,\#C] - need further polish}
 
One incident handler is tied to one incident type. The hit rate depends on the coverage of the incident type. If the team builds the handler for every alert type, then the coverage would be 100\%. 
 
 
 
\textbf{Q6. Root cause categories clarification? [\#B]}
 
We ask experienced engineers to set up the root cause categories, and there are XXX categories in our database. 
We admit that some categories may sound broad, but for the purpose of the incident classification, it is fine in the current setting. 
We will clarify that the LLM is predicting the incident root cause category with an explanation early in the paper.
 
 
\textbf{Q7. Does the prediction prompt require the developer's manual selection? [\#B]}
 
No. All parts of the prompt are generated automatically.
 
 

